You Don't Know My Favorite Color: Preventing Dialogue Representations from Revealing Speakers' Private Personas

Social chatbots, also known as chit-chat chatbots, evolve rapidly with large pretrained language models. Despite the huge progress, privacy concerns have arisen recently: training data of large language models can be extracted via model inversion attacks. On the other hand, the datasets used for training chatbots contain many private conversations between two individuals. In this work, we further investigate the privacy leakage of the hidden states of chatbots trained by language modeling which has not been well studied yet. We show that speakers' personas can be inferred through a simple neural network with high accuracy. To this end, we propose effective defense objectives to protect persona leakage from hidden states. We conduct extensive experiments to demonstrate that our proposed defense objectives can greatly reduce the attack accuracy from 37.6% to 0.5%. Meanwhile, the proposed objectives preserve language models' powerful generation ability.

==> tab-predict_sample.tex <==
\begin{table}[t]
\small
\begin{tabular}{p{0.95\linewidth}}%{l}
\toprule
\textbf{Dialog Context} \\
\textbf{Human A}: Hello. I am so tired from all of this studying.\\
\textbf{Human B}: Hello. I loved studying when i was in school.\\
\textbf{Human A}: I am still working towards my degree.\\
\textbf{Human B}: Keep going! After college I began building houses out of matches, haha.\\
\textbf{Human A}: LOL, I am going to be a history teacher. \\
\textbf{Human B}: I studied Greek. My dog that I rescued while in college proved more useful. \\
\textbf{Human A}: Me and my father were both in the military, so history is important to me. \\
\textbf{Human B}: \textcolor{orange}{My father loved history too, he and mother died in a plane crash.} \\
\midrule
\textbf{Persona Prediction}: \\
\textbf{LM}:  My parents died. \textcolor{green}{\textbf{\cmark}}\\
%my parents died in a plane crash
\textbf{LM+KL+MI}: My favorite color is blue. \textcolor{red}{\textbf{\xmark}}\\
\bottomrule
\end{tabular}
%Dialog Context \\
%\hline
%Speaker A: \\
\caption{One persona inference attack example.
The embeddings of the final utterance with orange color are used for inferring B's persona. 
}
\label{tab:inference sample}
\end{table}
